Privacy-preserving Analytics for Data Markets using MPC

Data markets have the potential to foster new data-driven applications and help growing data-driven businesses. When building and deploying such markets in practice, regulations such as the European Union's General Data Protection Regulation (GDPR) impose constraints and restrictions on these markets especially when dealing with personal or privacy-sensitive data. In this paper, we present a candidate architecture for a privacy-preserving personal data market, relying on cryptographic primitives such as multi-party computation (MPC) capable of performing privacy-preserving computations on the data. Besides specifying the architecture of such a data market, we also present a privacy-risk analysis of the market following the LINDDUN methodology.

==> Makefile <==
## please modify the following line for naming the end products (PDFs, ZIPs, ...)
PROJECTNAME = "KRArchitecture"

## -----------------------------------------
##       DO NOT EDIT BELOW THIS LINE
## -----------------------------------------

## Makefile from Karl Voit (Karl@Voit.net)

## some Makefile-hints taken from: 
## http://www.ctan.org/tex-archive/help/uk-tex-faq/Makefile


MAINDOCUMENTBASENAME = architecture
MAINDOCUMENTFILENAME = ${MAINDOCUMENTBASENAME}.tex
## COMMANDS:
PDFLATEX_CMD = pdflatex
BIBTEX_CMD = bibtex
#BIBTEX_CMD = biber
MAKEIDX_CMD = makeindex
DATESTAMP = `/bin/date +%Y-%m-%d`
DATESTAMP_AND_PROJECT = ${DATESTAMP}_${PROJECTNAME}
#PDFVIEWER = xpdf
PDFVIEWER = evince #acroread

#help
#helpThe main targets of this Makefile are:
#help	help	this help
.PHONY: help
help:
	@sed -n 's/^#help//p' < Makefile

#help	all	see "pdf"
.PHONY: all
all: pdf

#help	1       compiles the PDF once using pdflatex
.PHONY: 1 
1:
	${PDFLATEX_CMD} ${MAINDOCUMENTFILENAME}
	-mv ${MAINDOCUMENTBASENAME}.pdf ${PROJECTNAME}.pdf

#help	2       compiles the PDF twice using pdflatex
.PHONY: 2 
2:
	${PDFLATEX_CMD} ${MAINDOCUMENTFILENAME}
	${PDFLATEX_CMD} ${MAINDOCUMENTFILENAME}
	-mv ${MAINDOCUMENTBASENAME}.pdf ${PROJECTNAME}.pdf

#help	pdf	creates a pdf file using pdflatex
.PHONY: pdf
pdf:
	${PDFLATEX_CMD} ${MAINDOCUMENTFILENAME}
	-${BIBTEX_CMD} ${MAINDOCUMENTBASENAME}
	${PDFLATEX_CMD} ${MAINDOCUMENTFILENAME}
	${PDFLATEX_CMD} ${MAINDOCUMENTFILENAME}
	#-mv ${MAINDOCUMENTBASENAME}.pdf ${DATESTAMP_AND_PROJECT}.pdf
	-mv ${MAINDOCUMENTBASENAME}.pdf ${PROJECTNAME}.pdf

#help	wc	counts the words from the PDF generated
wc:	pdf
	pdftops ${PROJECTNAME}.pdf
	ps2ascii ${PROJECTNAME}.ps > ${PROJECTNAME}.txt
	wc -w ${PROJECTNAME}.txt
	#pdftops ${DATESTAMP_AND_PROJECT}.pdf
	#ps2ascii ${DATESTAMP_AND_PROJECT}.ps > ${DATESTAMP_AND_PROJECT}.txt
	#wc -w ${DATESTAMP_AND_PROJECT}.txt


# --------------------------------------------------------

#help	view	view the PDF-file
.PHONY: view
view: 
	${PDFVIEWER} ${PROJECTNAME}.pdf &
	#${PDFVIEWER} ${DATESTAMP_AND_PROJECT}.pdf

# --------------------------------------------------------


#help	clean	clean up temporary files
.PHONY: clean
clean: 
	-rm -r *.bcf *.run.xml _*_.* *~ *.aux *-blx.bib *.bbl ${MAINDOCUMENTBASENAME}.dvi *.ps *.blg *.idx *.ilg *.ind *.toc *.log *.log *.brf *.out *.lof *.lot *.gxg *.glx *.gxs *.glo *.gls *.tdo -f

#help	purge	cleaner than clean ;-)
.PHONY: purge
purge: clean
	-rm *.ps -f

#help	force	force rebuild next run
.PHONY: force
force:
	touch *tex

# TOOLS:

#help	zip	create ZIP-file
.PHONY: zip
zip: purge pdf clean
	zip -r ../${PROJECTNAME}_${TIMESTAMP}.zip *

#.PHONY: publish
#publish: templatedocu pdf clean
#	-rm 20*.pdf ${TEMPLATEDOCUFILE} -f
#	git status

#help	templatedocu	updates tex-files for the documentation of this template
#help			needs: echo, sed, grep
#.PHONY: templatedocu
#templatedocu:
#	grep "%doc%" template/preamble.tex | sed 's/^.*%doc% //' > ${TEMPLATEDOCUFILE}
#	grep "%doc%" template/mycommands.tex | sed 's/^.*%doc% //' >> ${TEMPLATEDOCUFILE}
#	grep "%doc%" template/typographic_settings.tex | sed 's/^.*%doc% //' >> ${TEMPLATEDOCUFILE}
#	grep "%doc%" template/pdf_settings.tex | sed 's/^.*%doc% //' >> ${TEMPLATEDOCUFILE}
#	echo "%%---------------------------------------%%" >>${TEMPLATEDOCUFILE}
#	echo "\printbibliography\end{document}" >>${TEMPLATEDOCUFILE}
#	${PDFLATEX_CMD} ${TEMPLATEDOCUFILE}
#	${PDFLATEX_CMD} ${TEMPLATEDOCUFILE}
#	${BIBTEX_CMD} ${TEMPLATEDOCUBASENAME}
#	${PDFLATEX_CMD} ${TEMPLATEDOCUFILE}


#end

architecture.pdf: architecture.tex dblp.bib bib.bib
	latexmk -f architecture.tex

cr.zip: architecture.pdf
	zip cr.zip \
		architecture.tex \
		architecture.pdf \
		dblp.bib \
		bib.bib \
		architecture.bbl \
		architecture.blg \
		llncs.cls \
		macros.tex \
		splncs04.bst \
		figures/linddun_steps.png \
		figures/diagrams_gliffy/architecture.pdf \
		figures/diagrams_gliffy/DFD_user_registration.pdf \
		figures/diagrams_gliffy/DFD_cloud_storage_compact.pdf

